Strong subalgebras and the Constraint Satisfaction Problem

In 2007 it was conjectured that the Constraint Satisfaction Problem (CSP) over a constraint language $\Gamma$ is tractable if and only if $\Gamma$ is preserved by a weak near-unanimity (WNU) operation. After many efforts and partial results, this conjecture was independently proved by Andrei Bulatov and the author in 2017. In this paper we consider one of two main ingredients of my proof, that is, strong subalgebras that allow us to reduce domains of the variables iteratively. To explain how this idea works we show the algebraic properties of strong subalgebras and provide self-contained proof of two important facts about the complexity of the CSP. First, we prove that if a constraint language is not preserved by a WNU operation then the corresponding CSP is NP-hard. Second, we characterize all constraint languages that can be solved by local consistency checking. Additionally, we characterize all idempotent algebras not having a WNU term of a concrete arity $n$, not having a WNU term, having WNU terms of all arities greater than 2. Most of the results presented in the paper are not new, but I believe this paper can help to understand my approach to CSP and the new self-contained proof of known facts will be also useful.

==> CSPProofsCopy.tex <==
\section{Constraint Satisfaction problem}

In this section we will demonstrate how 
strong subalgebras can be used to study the complexity of the  Constraint Satisfaction Problem 
for 
different constraint languages.

\subsection{CSP Dichotomy Conjecture}

%For a finite set $A$
%by $\mathcal R_{A}$ we denote the set of all 
%relations on $A$.
Suppose we have a 
finite set of relations $\Gamma\subseteq \mathcal R_{A}$, called 
\emph{a constraint language}.
%Note that 
%every $h$-ary relation on $A$ can be viewed as
%a predicate, that is, a
%mapping $A^{h}\rightarrow \{true,false\}$.
Recall that 
\emph{the Constraint Satisfaction Problem over the constraint language $\Gamma$},  denote by $\CSP(\Gamma)$, is the 
following decision problem:
given a formula
$$R_{1}(v_{1,1},\ldots,v_{1,n_{1}})
\wedge
\dots
\wedge
R_{s}(v_{s,1},\ldots,v_{1,n_{s}}),$$
where $R_{1},\dots,R_{s}\in \Gamma$, 
and $v_{i,j}\in \{x_{1},\dots,x_{n}\}$ for every $i,j$;
decide whether this formula is satisfiable.
We call each
$R_{i}(v_{i,1},\ldots,v_{i,n_{i}})$ \emph{a constraint}.

It is well known that many combinatorial problems can be expressed as $\CSP(\Gamma)$
for some constraint language $\Gamma$.
Moreover, for some sets $\Gamma$ the corresponding decision problem can be solved in polynomial time (tractable);
while for others it is NP-complete.
It was conjectured that
$\CSP(\Gamma)$ is either in P, or NP-complete \cite{FederVardi}.
In 2017, two independent proofs of these conjecture
(called the CSP Dichotomy Conjecture) appeared, 
and the characterization of the tractable constraint languages 
turned out to be very simple.
%An operation $f$ on a set $A$ is called \emph{a weak near-unanimity operation (WNU)} if it satisfies 
%$f(x,x,\ldots,x) = x$ and
%$f(y,x,\ldots,x) = f(x,y,x,\ldots,x) = \dots = f(x,x,\ldots,x,y)$
%for all $x,y\in A$.
%Then the CSP Dichotomy theorem can be formulated in the following nice way.

\begin{thm}\label{CSPDichotomyTHM}\cite{BulatovProofCSP,MyProofCSP,ZhukFOCSCSPPaper}
Suppose $\Gamma\subseteq R_{A}$ is a finite set of relations.
Then $\CSP(\Gamma)$ can be solved in polynomial time if there exists a WNU operation
preserving $\Gamma$;
$\CSP(\Gamma)$ is NP-complete otherwise.
\end{thm}

In this section we demonstrate how strong subalgebras
can be used to prove the 
hardness part of Theorem~\ref{CSPDichotomyTHM}, 
and to characterize all constraint languages $\Gamma$ 
such that $\CSP(\Gamma)$ can be solved by local consistency checking. 


\subsection{Reduction to a core}\label{ReductionToAcoreSubsection}

First, we need to show that it is sufficient to consider only idempotent case, that is the case when $\Gamma$ contains all the relations of the form $x=a$ for $a\in A$
(we call them \emph{constant relations}).
Suppose $f$ is a unary polymorphism of $\Gamma$, 
and $f(\Gamma)$ is a constraint language with domain $f(A)$
defined by $f(\Gamma) = \{f(R)\colon R\in \Gamma\}$.
It is easy to see that a CSP instance 
of $\CSP(\Gamma)$ is equivalent to 
the corresponding instance of $\CSP(f(\Gamma))$
where we replace each relation $R_{i}$ 
by $f(R_{i})$. So the following lemma holds.

\begin{lem}\label{ReductionToACore}\cite{jeavons1998algebraic}
Suppose $f$ is a unary polymorphism of $\Gamma$.
Then $\CSP(\Gamma)$ is polynomially equivalent to 
$\CSP(f(\Gamma))$.
\end{lem}
% (see \cite{CSPconjecture} for the details).
Thus, if there exists a unary polymorphism that is not a bijection, 
this polymorphism can be used to reduce the 
domain.

A constraint language is called \emph{a core} if every unary polymorphism of $\Gamma$ is a bijection.
It is not hard to show that if $f$ is a unary polymorphism of $\Gamma$ with minimal range,
then $f(\Gamma)$ is a core \cite{CSPconjecture}. Another important fact is that we can add all
constant relations to a core constraint language
without increasing the complexity of its $\CSP$.
First we will need an auxiliary fact.

\begin{lem}\label{QuantifierFreeDefinitionOfSigma}
Suppose $A=\{0,1,\dots,k-1\}$, $\Gamma\subseteq\mathcal R_A$
and 
$\algA = (A;\Pol(\Gamma))$.
Then $\Sg_{\algA^{k}}(
\{(0,1,\dots,k-1)\})$ has a quantifier-free pp-definition over $\Gamma$.
\end{lem}
\begin{proof}
Let us show that $\Sg_{\algA^{k}}(
\{(0,1,\dots,k-1)\})$ is defined by 
$$\sigma(z_{0},\dots,z_{k-1}) = \bigwedge_{R\in \Gamma, 
(a_1,\dots,a_{s})\in R} R(z_{a_1},z_{a_2},\dots,z_{a_s}).$$
By the definition, $(0,1,\dots,k-1)\in\sigma$. 
If $(b_0,b_1,\dots,b_{k-1})\in\sigma$, 
then the definition of $\sigma$ just says that the unary function $g(x) = b_x$ preserves every relation 
$R\in\Gamma$, and this is exactly what we need.
\end{proof}


\begin{thm}\label{addingIdempotency}\cite{CSPconjecture}
Let $\Gamma\subseteq\mathcal R_A$ be a core constraint language, and
$\Gamma' = \Gamma\cup \{x=a\mid a\in A\}$.
Then $\CSP(\Gamma')$ is polynomially reducible to $\CSP(\Gamma)$.
\end{thm}

\begin{proof}
Assume that 
$A =\{0,1,\dots,k-1\}$. 
Let $\algA = (A;\Pol(\Gamma))$
and $\sigma = \Sg_{\algA^{k}}(
\{(0,1,\dots,k-1)\})$.
By Lemma~\ref{QuantifierFreeDefinitionOfSigma}
%We know from the Galois connection between clones and relational clones that $\sigma$ is pp-definable over $\Gamma$.
$\sigma$ has a quantifier-free pp-definition over $\Gamma$.
Suppose we have an instance $\mathcal I'$ of 
$\CSP(\Gamma')$. 
Choose $k$ new variables 
$z_{0},\dots,z_{k-1}$ and replace every constraint 
$x=a$ by $x=z_{a}$. 
Also, add the pp-definition of the constraint 
$\sigma(z_{0},\dots,z_{k-1})$.
The obtained instance we denote by 
$\mathcal I$.
Let us show that 
$\mathcal I$ is equivalent to $\mathcal I'$.

$\mathcal I'\Rightarrow \mathcal I$.
To get a solution of $\mathcal I$ it is sufficient to take a solution of 
$\mathcal I'$ and put 
$z_{a} = a$ for every $a\in A$.

$\mathcal I\Rightarrow \mathcal I'$.
Consider a solution of $\mathcal I$.
Let $(z_{0},\dots,z_{k-1}) = 
(b_{0},\dots,b_{k-1})$ in this solution.
Since $(b_{0},\dots,b_{k-1})\in\sigma$ and $\Gamma$ is a core, 
there exists a unary bijective polymorphism 
$\varphi$ such that 
$\varphi(0,1,\dots,k-1) = 
(b_{0},b_{1},\dots,b_{k-1})$.
Composing $\varphi$ we can define a unary bijective polymorphism 
$\psi$ such that 
$\psi(b_{0},b_{1},\dots,b_{k-1}) = 
(0,1,\dots,k-1)$.
Applying $\psi$ to the solution of $\mathcal I$ 
we get a solution of $\mathcal I'$.
\end{proof}

Combining Lemma~\ref{ReductionToACore} and 
Theorem~\ref{addingIdempotency} we conclude that 
it is sufficient to consider only idempotent case to
prove the CSP Dichotomy Conjecture. 

\subsection{Hardness Result}

Note that the original proof of the following hardness result 
is a combination of \cite{CSPconjecture} and \cite{miklos}.
We will derive the hardness result from Theorem \ref{CharacterizationOfAWNUTHM}, which is 
very similar to the claim proved in \cite{miklos}.

\begin{thm}\cite{CSPconjecture,miklos}
Suppose $\Gamma$ does not have a WNU polymorphism, 
then 
$\CSP(\Gamma)$ is NP-hard.
\end{thm}

\begin{proof}
Consider a unary polymorphism $f$ of $\Gamma$ 
with a minimal range.
Then 
$f(\Gamma)$ is a core constraint language.
%and 
%by Lemma~\ref{ReductionToACore}, $\CSP(f(\Gamma))$ is 
%polynomially equivalent to $\CSP(\Gamma)$,
Put $\Gamma' = f(\Gamma)\cup\{x=a\mid a\in f(A)\}$.
By Lemma~\ref{ReductionToACore} and Theorem~\ref{addingIdempotency}, 
$\CSP(\Gamma)$ is polynomially equivalent $\CSP(\Gamma')$.
Let $B = f(A)$, and $\alg B = (B;\Pol(\Gamma'))$.
If $\Gamma'$ has a WNU polymorphism $w'$, then 
$w(x_{1},\dots,x_{m}) = 
w'(f(x_{1}),\dots,f(x_{m}))$ is a WNU polymorphism 
of $\Gamma$.
Since $\Gamma$ does not have a WNU polymorphism, 
neither do $\Gamma'$.
By Theorem~\ref{CharacterizationOfAWNUTHM}, there exists 
a WNU-blocker $R\in\Inv(\alg B)$.
By the Galois connection we know that 
$R$ is pp-definable over $\Gamma'$ 
(we also need the equality and empty relations but they can always be propagated out from the pp-definition of $R$).
Let us show that 
$\CSP(\Gamma')$ is NP-hard. 
Let $\mathrm{NAE}_3$ be the ternary relation on $\{0,1\}$ containing 
all tuples except for $(0,0,0)$ and $(1,1,1)$.
Consider an instance 
$\mathcal I$ of $\CSP(\{\mathrm{NAE}_3\})$, 
which is known to be an NP-hard problem \cite{Schaefer}.
Replace each $\mathrm{NAE}_3$-relation by $R$, then replace each $R$ by
its pp-definition over $\Gamma'$ (all existentially quantified variables are the new variables of the instance). The obtained instance is equivalent to $\mathcal I$, which proves that $\CSP(\Gamma')$ is NP-hard.
\end{proof}

\subsection{Cycle-consistency}

In this subsection we 
introduce the notion of cycle-consistency (similar to singleton-arc-consistency in \cite{kozik2016weak}) , which is a type of local consistency, 
and show that if a constraint language 
has a WNU polymorphism of every arity $n\ge 3$
then every cycle-consistent instance has a solution.
In Subsection \ref{whenccworkssubsection} we will argue that 
whenever the instance can be solved by local methods, 
it can be solved by local consistency checking.
For more information about 
notions of local consistency see 
\cite{bartokozikboundedwidth,kozik2016weak}.

We will need several definitions.
Here we assume that 
every variable $x$ has its own domain $D_{x}\subseteq A$. We also require each $D_{x}$ to be pp-definable over
the constraint language $\Gamma$
to guarantee that every operation from $\Pol(\Gamma)$ 
preserves $D_{x}$.
For an instance $\mathcal I$ by 
$\Var(\mathcal I)$ we denote the set of 
all variables appearing in $\mathcal I$.

For an instance $\mathcal I$ and a set of variables 
$(y_{1},\dots,y_{t})$ by
$\mathcal I(y_{1},\dots,y_{t})$ we denote the set of tuples
$(b_{1},\dots,b_{t})$ such that $\mathcal I$ 
has a solution with 
$y_{1} = b_{1},\dots,y_{t} = b_{t}$.
Thus, this expression can be viewed as a pp-definition of a relation of the arity $t$ over $\Gamma$.


We say that $z_{1}-C_{1}-z_{2}-\dots - C_{l-1}-z_{l}$ is
\emph{a path} in a CSP instance $\mathcal I$ if $z_{i},z_{i+1}$ are in the scope of the constraint $C_{i}$ for every $i\in[l]$.
We say that \emph{a path $z_{1}-C_{1}-z_{2}-\dots -C_{l-1}-z_{l}$  connects $b$ and $c$}
if there exists $a_{i}\in D_{z_{i}}$ for every $i\in[l]$
such that
$a_{1} = b$, $a_{l} = c$, and
the projection of $C_{i}$ onto $z_{i}, z_{i+1}$
contains the tuple $(a_{i},a_{i+1})$.
A CSP instance is called \emph{1-consistent} if 
the projection of any constraint $C$ onto any of its variable 
$x$ is equal to $D_{x}$.
A CSP instance is called \emph{cycle-consistent} if
it is 1-consistent and 
for every variable $z$ and $a\in D_{z}$
any path starting and ending with $z$ in $\mathcal I$
connects $a$ and $a$.

An instance is called a \emph{tree-instance}
if there is no a path
$z_{1}-C_{1}-z_{2}-\dots -z_{l-1}-C_{l-1}-z_{l}$
such that $l\ge 3$, $z_{1} = z_{l}$, and all the constraints $C_{1},\ldots,C_{l-1}$ are different.
A instance $\mathcal J$ is called 
\emph{a covering} of an instance 
$\mathcal I$ if there 
exists a mapping 
$\psi:\Var(\mathcal J)\to \Var(\mathcal I)$
such that
for every constraint $R(x_{1},\ldots,x_{n})$ of $\mathcal J$ the expression
$R(\psi(x_{1}),\ldots,\psi(x_{n}))$ 
is a constraint of $\mathcal I$.
%For the simplicity of the notations we assume that if 
%$y\in\Var(\mathcal I)\cap \Var(\mathcal J)$ then 
%$\psi(y) = y$.
We say that a covering is 
a \emph{tree-covering} if it is a tree-instance.
An important property of a tree-covering 
$\Upsilon$
of a 1-consistent instance 
is that 
$\Upsilon(y) = D_{y}$ for every variable $y$, 
that is we can choose any value for the variable $y$ 
a extend this value to a solution of $\Upsilon$.


A mapping $D^{(\top)}\colon\Var(\mathcal I)\to A$ is called 
a reduction of the instance $\mathcal I$ if 
$D^{(\top)}_{x}\subseteq D_{x}$ 
and $D^{(\top)}_{x}$ is pp-definable over $\Gamma$ for every $x\in\Var(\mathcal I)$. 

We usually denote reductions by $D^{(1)},D^{(j)},D^{(\top)},D^{(\bot)}$.
We say that 
$D^{(\bot)}\le D^{(\top)}$ if 
$D^{(\bot)}_{y}\subseteq D^{(\top)}_{y}$ for every $y$.
We say that a reduction $D^{(\top)}$ is \emph{empty}
if $D_{y}^{(\top)}=\varnothing$ for every variable $y$.
For an instance $\mathcal I$
by $\mathcal I^{(\top)}$ we denote the instance 
obtained from $I$ by 
\begin{enumerate}
    \item replacing the domain of each variable $x$ by
    $D^{(\top)}_{x}$, and
    \item replacing every constraint $R(x_{1},\dots,x_{n})$
    by $R'(x_{1},\dots,x_{n})$, where 
    $R' = R\cap (D^{(\top)}_{x_1}\times\dots\times D^{(\top)}_{x_n})$.
\end{enumerate}
Note that 
the constraint relations of $\mathcal I^{(\top)}$
are not longer from $\Gamma$, but they are always pp-definable over $\Gamma$.
A reduction $D^{(\top)}$ of an instance $\mathcal I$ 
is called \emph{1-consistent} if 
the instance $\mathcal I^{(\top)}$ is 1-consistent.


Note that any reduction of an instance can be naturally extended 
to a covering of the instance, 
thus we assume that any reduction is automatically defined on 
a covering.

The next Lemma has its roots in Theorem 20 from \cite{FederVardi},
where the authors proved that bounded width 1
is equivalent to tree duality. 

\begin{lem}\label{ConstraintPropagation}
Suppose $D^{(\top)}$ is a reduction of an instance $\mathcal I$ and
$D^{(\bot)}$ is a maximal 1-consistent reduction of $\mathcal I^{(\top)}$.
Then for every variable $y$ of $\mathcal I$ there exists a tree-covering  $\Upsilon_{y}$ of $\mathcal I$
such that
$\Upsilon_{y}^{(\top)}(y)$ defines $D_{y}^{(\bot)}$.
\end{lem}

\begin{proof}
The proof is based on the constraint propagation procedure.
We start with an empty instance $\Upsilon_{y}$ (empty tree-covering) for every variable $y$ of $\mathcal I$, 
we iteratively change these tree-coverings to obtain
tree-coverings defining the reduction $D^{(\bot)}$ as required.
At the beginning 
the 
reduction $D^{(\bot)}$
is defined by 
$D^{(\bot)}_{y} := \Upsilon_{y}^{(\top)}(y) = D^{(\top)}_{y}$
for every variable $y$.

If at some step the reduction $D^{(\bot)}$ is 1-consistent,
then we are done. 
Otherwise, consider a constraint $R(z_{1},\dots,z_{l})$ of $\mathcal I$ that breaks 1-consistency of $\mathcal I^{(\bot)}$, which means that 
the restriction of the variables $z_{1},\ldots,z_{l}$ to 
the sets $D^{(\bot)}_{z_{1}},\dots,D^{(\bot)}_{z_{1}}$
implies a stronger restriction of some variable $z_{i}$.
We change the tree-covering $\Upsilon_{z_{i}}$
by
$\Upsilon_{z_{i}}:= R(z_{1},\dots,z_{l})\wedge \Upsilon_{z_{1}}\wedge\dots\wedge\Upsilon_{z_{l}}$,
where we rename the variables of 
$\Upsilon_{z_{1}},\dots,\Upsilon_{z_{l}}$ so that 
they did not have common variables inside the new definition 
of $\Upsilon_{z_{i}}$,
and $\Upsilon_{z_{i}}$ stayed a tree-covering.
As a result we reduce 
the domain $D^{(\bot)}_{z_{i}}$ to 
$\Upsilon_{z_{i}}^{(\top)}(z_{i})$.

Since our instance is finite and every time we reduce some domain, this procedure will stop eventually giving us the required reduction $D^{(\bot)}$.

It remains to explain why the reduction 
$D^{(\bot)}$ is maximal.
Consider  a 1-consistent reduction 
$D^{(1)}\le D^{(\top)}$.
Since $\Upsilon_{y}$ is a tree-covering,
%and $D^{(1)}$ is 1-consistent, 
we have 
$\Upsilon_{y}^{(1)}(y) = D_{y}^{(1)}$.
Hence 
$D_{y}^{(1)} = \Upsilon_{y}^{(1)}(y)
\subseteq \Upsilon_{y}^{(\top)}(y)
=D_{y}^{(\bot)}$.
\end{proof}

The following theorem was originally proved in \cite{kozik2016weak}.

\begin{thm}\label{CycleConsistencyImpliesSolutionIdemp}
Suppose $\Gamma\subseteq \mathcal R_{A}$ is a constraint language containing all constant relations and having a WNU polymorphism of every arity $n\ge 3$, and 
$\mathcal I$ is a cycle-consistent instance of $\CSP(\Gamma)$.
Then $\mathcal I$ has a solution.
\end{thm}

\begin{proof}
Let $\algA = (A;\Pol(\Gamma))$.
Since every domain $D_{x}$ has a pp-definition over $\Gamma$, it is a subuniverse of the algebra $\algA$.
Hence, we may consider a subalgebra 
$\alg D_{x}\le \algA$ for every variable $x$ of $\mathcal I$.

The idea of the proof is to build a sequence of 
1-consistent reductions 
$D^{(0)}\ge D^{(1)}\ge \dots\ge D^{(t)}$ 
of the instance $\mathcal I$
such that 
\begin{enumerate}
\item[(1)] $D^{(0)}_{y} = D_{y}$ for every $y\in\Var(\mathcal I)$;
\item[(2)] $|D^{(t)}_{y}| = 1$ for every $y\in\Var(\mathcal I)$;
\item[(3)] $D^{(i)}_{y}$ is a strong subuniverse of 
$\alg D^{(i-1)}_{y}$ of type $\mathcal T_{i}$ for every $y\in\Var(\mathcal I)$ and $i\in\{1,2,\dots,t\}$.
\end{enumerate}
Obviously, 
the 1-consistent reduction 
$D^{(t)}$ gives us a solution of the instance.

Assume that we already have 
reductions 
$D^{(0)}, D^{(1)},\dots,D^{(s)}$.
Let us show how to build the next reduction.

Choose a variable $x$ such that  
$|D_{x}^{(s)}|>1$.
%By Theorem~\ref{ExistsStrongSubalgebraTHM} one of the five cases holds.
%Fourth case cannot happen because we cannot have an idempotent 
%WNU of arity 
%Apply 
%Since $D_{x}^{(s)}$ is a subuniverse of $A$,
By Theorem~\ref{CharacterizationOfALLWNUTHM} there should be a nontrivial strong subalgebra $B$ of $\alg D_{x}^{(s)}$ of a type $\mathcal T_{s+1}$. 
Most likely, if we just reduce 
$D_{x}^{(s)}$ to $B$ then the obtained instance 
will not be 1-consistent.
Nevertheless, we can reach 1-consistency.

By $D^{(\top)}$ we denote the 
reduction that coincides with 
$D^{(s)}$ on all variables but $x$ and $D_{x}^{(\top)} = 
B$.

By $D^{(\bot)}$ we denote a maximal 1-consistent reduction of $\mathcal I^{(\top)}$, which theoretically can be empty.
By Lemma~\ref{ConstraintPropagation} 
for every variable $y\in\Var(\mathcal I)$ 
there exists a tree-covering $\Upsilon_{y}$ of $\mathcal I$
such that $\Upsilon_{y}^{(\top)}(y)$ defines 
$D_{y}^{(\bot)}$.
We consider two cases.

Case 1. The reduction $D^{(\bot)}$ is empty,
then the instance $\Upsilon_{y}^{(\top)}$ does not have a solution.
We will show that this case cannot happen.
To simplify our notations we put $D^{(s+1)} = D^{(\top)}$. 
Let $X$ be the set of variables from $\Upsilon_{y}$ that are mapped to $x$ in the definition of the covering $\Upsilon_{y}$.
We know that $\Upsilon_{y}^{(s)}$ does not have a solution 
such that all of these variables are from $B$.
Choose a minimal set $\{x_{1},\dots,x_{\ell}\}\subseteq X$ of variables we need to restrict to $B$ so that 
$\Upsilon_{y}^{(s)}$ has no solutions.
Let $\Upsilon_{y}^{(s)}(x_{1},\dots,x_{\ell})$ define 
a relation $R$.
Then $R$ is a $B$-essential relation.
Since the instance $\mathcal I^{(s)}$ is 
1-consistent and 
$\Upsilon_{y}$ is a tree-covering of 
$\mathcal I$, the relation $R\le D_{x}^{(s)}\times \dots\times D_{x}^{(s)}$ is subdirect
and $\ell\ge 2$. 

By Theorem \ref{CommonPropertiesThm}(3),
$\mathcal T_{s+1}$ cannot be an absorbing type and 
$\ell=2$.
Let $\Var(\Upsilon_{y}) =
\{x_{1},x_{2},y_{1},\dots,y_{u}\}$
and $S$ be the solution set of 
$\Upsilon_{y}$, that is a relation defined by 
$\Upsilon_{y}(x_{1},x_{2},y_{1},\dots,y_{u})$.
Since $\mathcal I^{(i)}$ is 1-consistent for any $i\le s$ and 
$\Upsilon_{y}$ is a tree-covering, 
the relation $S^{(i)}$ is subdirect.

For $0\le i, j,k\le s+1$ put
%\begin{align*}
$
S_{i,j,k}= S\cap (D_{x_{1}}^{(i)}\times D_{x_{2}}^{(j)}\times D_{y_{1}}^{(k)}\times\dots\times D_{y_{u}}^{(k)})
$.
%\end{align*}

%For 
%$S_{i,j}= S\cap& (D_{x_{1}}^{(i)}\times D_{x_{2}}^{(i)}\times D_{y_{1}}^{(j)}\times\dots\times D_{y_{t}}^{(j)})$.
%\end{align*}

Let us show by induction on $i$ that  
$S_{i,i,k+1}$ is a strong subuniverse of 
$S_{i,i,k}$
for any $0\le k\le i\le s$.
For $i=k$ this follows from 
Theorem~\ref{CommonPropertiesThm}(1) and the fact that $S^{(k)}$ is subdirect.
Let us prove the induction step assuming that 
$S_{i,i,k+1}$ is a strong subuniverse of 
$S_{i,i,k}$.
Since $S^{(i)}$ is subdirect,
Theorem~\ref{CommonPropertiesThm}(1) implies that $S_{i+1,i+1,k}$ is a strong subuniverse of 
$S_{i,i,k}$.
Then by Lemma~\ref{PCBsub}, 
we obtain that $S_{i+1,i+1,k}\cap S_{i,i,k+1} = S_{i+1,i+1,k+1}$
is a strong subuniverse of $S_{i+1,i+1,k}$.
Thus, $S_{i,i,k+1}$ is a strong subuniverse of 
$S_{i,i,k}$
for any $0\le k\le i\le s$.

%Since $\mathcal I^{(i)}$ is 1-consistent for any $i\le s$,
%$S^{(i)}$ is subdirect.
%Then by Lemma~\ref{PCBrel}
%$S_{i+1,i,k}$ and $S_{i,i+1,k}$ are strong subuniverses of 
%$S_{i,i,k}$ for $i\le k$.


Since $R\cap B^{2}=\varnothing$, 
we have $S_{s+1,s+1,s} = \varnothing.$
Since 
$\mathcal I$ is cycle-consistent,
the path from $x_1$ to $x_2$ in $\Upsilon_{y}$ 
connects any $a\in D_{x}^{(s+1)}$ with $a$.
Therefore. $S_{s+1,s+1,0}\neq \varnothing$.
Choose a minimal $k<s$ %\in\{0,1,\dots,s-1\}$ 
such that
$S_{s+1,s+1,k+1} = \varnothing.$
Thus, we have 
\begin{equation}\label{ThreeIntersection}
S_{s+1,s+1,k+1} = S_{s+1,s,k}\cap S_{s,s+1,k}\cap S_{s,s,k+1}
=\varnothing
\end{equation}
We already proved that 
$S_{s,s,k+1}$ is 
a strong subuniverse of $S_{s,s,k}$.
Since $S^{(s)}$ is subdirect, 
Theorem~\ref{CommonPropertiesThm}(1) implies that
$S_{s+1,s,k}$ and $S_{s,s+1,k}$ are strong subuniverses of 
$S_{s,s,k}$.
Thus, in (\ref{ThreeIntersection}) we 
have an intersection of three
strong subuniverses 
of $S_{s,s,k}$.

Since $k$ was chosen minimal, 
$S_{s+1,s+1,k}=S_{s+1,s,k}\cap S_{s,s+1,k}$ is not empty.
Since $S^{(s)}$ is subdirect,
$S_{s,s+1,s}\neq \varnothing$ and $S_{s+1,s,s}\neq \varnothing$.
Therefore 
$S_{s,s+1,k+1} = S_{s,s+1,k}\cap S_{s,s,k+1}\neq \varnothing$
and 
$S_{s+1,s,k+1} = S_{s+1,s,k}\cap S_{s,s,k+1}\neq \varnothing$.
Thus, the intersection of any two 
strong subuniverses in (\ref{ThreeIntersection}) 
is not empty.
Since %$\mathcal T_{s+1}$ is not a binary absorbing type,
$S_{s+1,s,k}$ is not a binary absorbing subuniverse, 
we get a contradiction
with Theorem~\ref{PCBint}.
%If the type $\mathcal T_{s+1}$ is an absorbing type, 
%Theorem~\ref{StrongSubalgebraEssential} 
%contradicts the fact that 
%$S_{s,s+1,k+1}\cap S_{s+1,s,k+1}=S_{s+1,s+1,k+1}=\varnothing.$
%Otherwise, w
%cont

Case 2. The reduction $D^{(\bot)}$ is not empty.
Put $D^{(s+1)} = D^{(\bot)}$.
Let $\Var(\Upsilon_{y}) = 
\{y,x_{1},\dots,x_{s}\}$ 
and 
$R_{y}$ be defined by 
$\Upsilon_{y}^{(s)}(y,x_{1},\dots,x_{s})$.
Since 
$\mathcal I^{(s)}$ is 1-consistent, 
the relation $R_{y}$ is subdirect.
We know that 
$D_{y}^{(s+1)} = %\Upsilon_{y}^{(\top)}(y) = 
\proj_{1}(R_{y}\cap (D_{y}^{(\top)}\times 
D_{x_{1}}^{(\top)}\times \dots\times D_{x_{s}}^{(\top)}))$.
By 
Theorem~\ref{CommonPropertiesThm}(2),
$D_{y}^{(s+1)}$
is a strong subuniverse of $D_{y}^{(s)}$ of type $\mathcal T_{s+1}$.
Thus, we proved that the new reduction $D^{(s+1)}$ 
satisfies condition (3), and we made our sequence of reductions longer.
\end{proof}

\subsection{An algorithm for cycle-consistency checking}

\newcommand{\Changed}{\mbox{Changed}}
\newcommand{\Solve}{\mbox{Solve}}
\newcommand{\Reduce}{\mbox{Reduce}}
\newcommand{\Output}{\mbox{Output}}
\newcommand{\CheckCycleConsistency}{\mbox{\textsc{SolveCC}}}



The cycle-consistency is a local property and it can be checked in polynomial time. 
Moreover, we can either find a cycle-consistent reduction of
the instance, or prove that it has no solutions.
Below we present the function 
$\CheckCycleConsistency$ doing this
for a CSP instance $\mathcal I$ (see the pseudocode). %$\CheckCycleConsistency$
%To do this it is sufficient to use constraint propagation providing a variant of (2,3)-consistency (see the pseudocode).
%We assume that we have an instance $\mathcal I$ 
%whose variables are $x_{1},\dots,x_{n}$.
First, for every pair of different variables $(u,v)$ we consider the intersections of projections of all constraints onto these variables.
The corresponding relation we denote by $R_{u,v}$.
Put $R_{u,u} = \{(a,b)\mid a=b\in R_{u}\}$, where 
$R_{u}$ is the intersection of the projections 
of all constraints on $u$.
Then, for every $u,v,w\in\Var(\mathcal I)$
we iteratively replace
$R_{u,v}$ by $R_{u,v}' = R_{u,v}\cap (R_{u,w}\circ R_{w,v})$,
where 
$R_{u,w}\circ R_{w,v}$ is the composition of binary relations, 
that is 
$(R_{u,w}\circ R_{w,v})(x,y)  = \exists  z \; R_{u,w}(x,z)\wedge R_{w,v}(z,y).$
We repeat this procedure while we can change some $R_{u,v}$.

In the end we may have two situations. 
If all $R_{u,u}$ are empty, then 
the function returns \mbox{``No solution"}.
Otherwise it returns \mbox{``Ok"}.
The following lemma explains the meaning of these answers.
 
\begin{lem}\label{ProofCycleConsistencyFunction}
If the function 
$\CheckCycleConsistency$ returns 
\mbox{``Ok"} then 
the reduction 
$D^{(\top)}$, defined by 
$D^{(\top)}_{y} = \proj_{1}(R_{y,y})$, is cycle-consistent,
if it returns \mbox{``No solution"}
then the instance has no solutions.
\end{lem}
\begin{proof}
Assume that the functions returned 
\mbox{``Ok"}. 
Since in the end of the algorithm
$R_{u,u}\circ R_{u,v}\supseteq R_{u,v}$ and 
$R_{u,v}\circ R_{v,u}\supseteq R_{u,u}$, 
we have 
$\proj_{1}(R_{u,v})
=\proj_{1}(R_{u,u})$
for every $u$.
Hence the reduction $D^{(\top)}$ is 1-consistent.
Let us prove the cycle-consistency.
Consider a path
$u_{1}-C_{1}-u_{2}-\dots-u_{\ell-1}-C_{\ell-1}-
u_{\ell}$
starting and ending 
with $u_{1}=u_{\ell}$. 
Since the projection 
of $C_{j}$ onto $u_{j},u_{j+1}$ 
contains $R_{u_{j},u_{j+1}}$ for every $j$, 
it is sufficient to prove 
that 
$$R_{u_1,u_\ell}\subseteq 
R_{u_{1},u_{2}}\circ 
R_{u_{2},u_{3}}\circ 
\dots
\circ 
R_{u_{\ell-1},u_{\ell}}.$$
Here we used the fact that the composition of binary relations is transitive (as follows from the definition.
Since the function stopped, 
$R_{u,v}\subseteq R_{u,w}\circ R_{w,v}$ 
for all $u,v,w$. 
Thus, in the right-hand  side we first replace 
$R_{u_{1},u_{2}}\circ 
R_{u_{2},u_{3}}$ by $R_{u_1,u_3}$, 
then replace $R_{u_{1},u_{3}}\circ 
R_{u_{3},u_{4}}$ by $R_{u_1,u_4}$, and so on.
Finally we will get the required condition.

Assume that the function 
returns \mbox{``No solution"}. 
Since all the constraints 
$R_{u,v}(u,v)$ were derived from the original constraints, they should hold on any solution.
Then if $R_{u,u}$ is empty, then 
the instance has no solutions.
\end{proof}



\begin{algorithm}
\begin{algorithmic}[1]
\Function{\CheckCycleConsistency}{$\mathcal I$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\mathcal I$}
    \For{$u,v\in\Var(\mathcal I)$} 
    \Comment{Calculate binary projections $R_{u,v}$}
        \State{$R_{u,v} := D_{u}\times D_{v}$}
        \For{$C\in\mathcal I$}        
            \State{$R_{u,v} :=R_{u,v}\cap \proj_{u,v} C$}
            %\Comment{$\proj_{x_i,x_j} C$ is the projection 
            %of $C$ onto $x_{i},x_{j}$}
        \EndFor
    \EndFor
    \Repeat \Comment{Propagate constraints to reduce  $R_{i,j}$}
        \State{$\Changed:= false$}
        \For{$u,v,w\in\Var(\mathcal I)$} 
            \State{$R_{u,v}'
            =R_{u,v}\cap (R_{u,w}\circ R_{w,v})$}
            \If{$R_{u,v} \neq R_{u,v}'$}
                \State{$R_{u,v}:=R_{u,v}'$}
                \State{$\Changed:= true$}               
            \EndIf
        \EndFor
    \Until{$\neg\Changed$} \Comment{We cannot reduce $R_{u,v}$ anymore}
    \State{Choose $u\in\Var(\mathcal I)$}
    \If{$R_{u,u}=\varnothing$}
        \Return{``No solution"}
    \Else{
        \Return{\mbox{``Ok"}}
        }
    \EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\begin{algorithmic}[1]
\Function{\CheckCycleConsistency}{$\mathcal I$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\mathcal I$}
    \For{$u\in\Var(\mathcal I)$} 
        \State{$D^{(\top)}_{u}:= D_{u}$}
        \Comment{We start with a trivial reduction $D^{(\top)}$}
    \EndFor
    \For{$u,v\in\Var(\mathcal I)$} 
    
    \Comment{Calculate binary projections $R_{u,v}$}
        \State{$R_{u,v} := D_{u}\times D_{v}$}
        \For{$C\in\mathcal I$}        
            \State{$R_{u,v} :=R_{u,v}\cap \proj_{u,v} C$}
            %\Comment{$\proj_{x_i,x_j} C$ is the projection 
            %of $C$ onto $x_{i},x_{j}$}
        \EndFor
    \EndFor
    \Repeat \Comment{Propagate constraints to reduce  $R_{i,j}$}
        \State{$\Changed:= false$}
        \For{$u,v,w\in\Var(\mathcal I)$} 
            \State{$R_{u,v}'
            =R_{u,v}\cap (R_{u,w}\circ R_{w,v})$}
            \If{$R_{u,v} \neq R_{u,v}'$}
                \State{$R_{u,v}:=R_{u,v}'$}
                \State{$\Changed:= true$}               
            \EndIf
        \EndFor
    \Until{$\neg\Changed$} \Comment{We cannot reduce $R_{u,v}$ anymore}
    \State{Choose $u\in\Var(\mathcal I)$}
    \If{$R_{u,u}=\varnothing$}
        \Return{``No solution"}
    \Else{
        \Return{\mbox{``Ok"}}
        }
    \EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\begin{algorithmic}[1]
\Function{\CheckCycleConsistency}{$\mathcal I$}
\State{\textbf{Input:} CSP($\Gamma$) instance $\mathcal I$}
    \For{$u\in\Var(\mathcal I)$} 
        \State{$D^{(\top)}_{u}:= D_{u}$}
        \Comment{We start with a trivial reduction $D^{(\top)}$}
    \EndFor
    \Repeat \Comment{Propagate constraints to reduce}    
    \For{$u,v\in\Var(\mathcal I)$} 
    
    \Comment{Calculate binary projections $R_{u,v}$}
        \State{$R_{u,v} := D_{u}\times D_{v}$}
        \For{$C\in\mathcal I$}        
            \State{$R_{u,v} :=R_{u,v}\cap \proj_{u,v} C$}
            %\Comment{$\proj_{x_i,x_j} C$ is the projection 
            %of $C$ onto $x_{i},x_{j}$}
        \EndFor
    \EndFor
    \Repeat \Comment{Propagate constraints to reduce  $R_{i,j}$}
        \State{$\Changed:= false$}
        \For{$u,v,w\in\Var(\mathcal I)$} 
            \State{$R_{u,v}'
            =R_{u,v}\cap (R_{u,w}\circ R_{w,v})$}
            \If{$R_{u,v} \neq R_{u,v}'$}
                \State{$R_{u,v}:=R_{u,v}'$}
                \State{$\Changed:= true$}               
            \EndIf
        \EndFor
    \Until{$\neg\Changed$} \Comment{We cannot reduce $R_{u,v}$ anymore}
    \For{$u\in\Var(\mathcal I)$} 
    \State{$D^{(\bot)}_{u}:= \proj_{1}(R_{u,u})$}
    \Comment{We start with a trivial reduction $D^{(\top)}$}
    \EndFor
    \Until{$D^{(\top)}=D^{(\bot)}$} \Comment{We cannot reduce $R_{u,v}$ anymore}
    \If{$D^{\top}$ is empty}
        \Return{``No solution"}
    \Else{
        \Return{\mbox{``Ok"}}
        }
    \EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}


Let us check that the algorithm is actually polynomial.
In the function 
$\CheckCycleConsistency$
we go through the \textbf{repeat} loop 
at most $2^{|A|^{2}}\cdot |\Var(\mathcal I)|^{2}$ times, 
because every time we change at least one relation $R_{u,v}$, which is binary, 
and we have $|\Var(\mathcal I)|^{2}$ of them.
Thus, the function works in polynomial time.

\subsection{When Cycle-consistency solves CSP}\label{whenccworkssubsection}

In this section we characterize all the constraint languages for which the cycle-consistency 
guarantees the existence of a solution and, therefore, 
the function $\CheckCycleConsistency$ solves $\CSP(\Gamma)$.

We will prove a general result for the nonidempotent case, that is why we need to repeat the construction we did in Subsection \ref{ReductionToAcoreSubsection}.
Again we assume that 
$A = \{0,1,\dots,k-1\}$.
Suppose $\Gamma\subseteq\mathcal R_{A}$ is a constraint language, 
$f$ is a unary polymorphism with the minimal range. 
Then $f(\Gamma)$ is the constraint language with domain $f(A)$
defined by $f(\Gamma) = \{f(R)\colon R\in \Gamma\}$.
Let 
$\Gamma' = f(\Gamma)\cup \{x=a\mid a\in f(A)\}$.
As we know from Lemma~\ref{ReductionToACore}
and Theorem \ref{addingIdempotency}
the problems 
$\CSP(\Gamma)$, $\CSP(f(\Gamma))$, 
and $\CSP(\Gamma')$ are polynomially equivalent.
Recall how we build an instance of $\CSP(\Gamma)$ 
from the instance of 
$\CSP(\Gamma')$.
Suppose we have an instance $\mathcal I'$ 
of $\CSP(\Gamma')$.
First, to get an instance $\mathcal I_{f}$ over $f(\Gamma)$ we add
the quantifier-free pp-definition of the relation 
$\sigma(z_{0},\dots,z_{k-1})$ over $f(\Gamma)$
(see the proof of Theorem \ref{addingIdempotency}
and Lemma~\ref{QuantifierFreeDefinitionOfSigma}),
and replace every constraint 
$(x=a)$ by $x=z_{a}$.
To get an instance $\mathcal I$ of $\CSP(\Gamma)$ we just replace every constraint relation 
$f(R)$ by $R$.
Thus we have a mapping, which we denote by $\Sigma$, 
that assigns an instance of $\CSP(\Gamma)$ to an instance of
$\CSP(\Gamma')$.
First, we show that 
$\CheckCycleConsistency$ works identically on 
$\Sigma(\mathcal I')$ and $\mathcal I'$

\begin{lem}\label{CheckConsistencyWorksTheSame}
Suppose %$\mathcal I = \Sigma(\mathcal I')$ and 
the function $\CheckCycleConsistency$ returns 
\mbox{``Ok"} on $\mathcal I'$, 
then it returns \mbox{``Ok"} on $\Sigma(\mathcal I')$.
\end{lem}

\begin{proof}
Suppose $\mathcal I = \Sigma(\mathcal I')$.
Since 
$\CheckCycleConsistency$ returns 
\mbox{``Ok"} on $\mathcal I'$, 
it stops
with nonempty relations $S_{u,v}$ 
for all variables $u,v\in\Var(\mathcal I')$, where $S_{u,v}$ is the value
of $R_{u,v}$
if we launch
$\CheckCycleConsistency$ on $\mathcal I'$.
Additionally, we assign
$S_{u} = \proj_{1}(S_{u,u})$, 
$S_{u,z_{i}} = S_{u}\times \{i\}$ 
$S_{z_{i},z_{j}} = \{i\}\times\{j\}$.
Thus, we defined $S_{u,v}$ for all 
variables 
$u,v\in\Var(\mathcal I)$.
Now, we argue that 
if we launch $\CheckCycleConsistency$ on $\mathcal I$, then
$R_{u,v}\supseteq S_{u,v}$ for 
all variables $u,v\in\Var(\mathcal I)$.
It is obviously true at the beginning.

Since $\CheckCycleConsistency$ stopped with 
$S_{u,v}$, we have 
$S_{u,v} \subseteq  S_{u,w}\circ S_{w,v}$, 
for all $u,v,w\in\Var(\mathcal I')$.
If one of the variables is $z_{i}$ then the same condition holds. Recursively, we can show that 
the property $R_{u,v}\supseteq S_{u,v}$ keeps
when we execute $\CheckCycleConsistency$ on $\mathcal I$.
Thus, we always have 
$R_{u,v}\supseteq S_{u,v}\neq \varnothing$, hence
$\CheckCycleConsistency$ returns 
\mbox{``Ok"} on $\mathcal I$.
\end{proof}

Second, we generalize Theorem~\ref{CycleConsistencyImpliesSolutionIdemp} for the nonidempotent case.

\begin{thm}\label{CycleConsistencyImpliesSolutionNonidemp}
Suppose $\Gamma\subseteq \mathcal R_{A}$ is a constraint language having a WNU polymorphism of every arity $n\ge 3$, and 
$\mathcal I$ is a cycle-consistent instance of $\CSP(\Gamma)$.
Then $\mathcal I$ has a solution.
\end{thm}
\begin{proof}
For every $n\ge 3$ the constraint language $\Gamma$ has a 
WNU polymorphism of arity $n$.
Then $f(w(x_{1},\dots,x_{n}))$ is a WNU 
polymorphism of $f(\Gamma)$.
To make this polymorphism idempotent
consider 
the function $g$ defined by
$g(x) = f(w(x,x,\dots,x))$, which is a bijection on $f(A)$
because $f$ has a minimal range.
Composing $g$ we can get $h$ such that 
$h(g(x)) = x$ on $f(A)$.
Therefore, 
$h(g(w(x_{1},\dots,x_{n})))$ gives us 
an $n$-ary idempotent polymorphism of $f(\Gamma)$, 
which is also a polymorphism 
of $\Gamma'$.
Thus, we proved that $\Gamma'$ has an idempotent 
WNU polymorphism of any arity $n\ge 3$.

Consider the instance 
$\mathcal I_{0}$ of $\CSP(f(\Gamma))$
that is obtained from $\mathcal I$ by replacing of every constraint relation $R$ by $f(R)$.
Note that this is also an instance of $\CSP(\Gamma')$. 
Let us show that 
$\mathcal I_{0}$ is cycle-consistent.
Consider a path in $\mathcal I_{0}$
$$u_{1}-f(C_{1})-u_{2}-\dots-u_{\ell-1}-f(C_{\ell-1})-
u_{\ell}$$
starting and ending 
with $u_{1}=u_{\ell}$. 
Consider an element $b\in f(A)$.
Let $b = f(c)$ for some element $c\in A$.
Since $\mathcal I$ is cycle-consistent 
the same path in $\mathcal I$ connects 
$c$ and $c$. To connect $b$ and $b$ in $\mathcal I_{0}$ 
we apply $f$ to the assignment of each variable.
Thus, the instance 
$\mathcal I_{0}$ is cycle-consistent.
By Theorem~\ref{CycleConsistencyImpliesSolutionIdemp},
it has a solution.
Since $f(R)\subseteq R$ for every $R\in\Gamma$, it is also a solution of the original instance 
$\mathcal I$.
\end{proof}




\begin{lem}\label{CheckCycleConsistencyFailExample}
Suppose a $p$-WNU-blocker $R$ is pp-definable over $\Gamma\subseteq \mathcal R_{A}$
and $\Gamma$ contains all constant relations.
Then there exists an instance 
$\mathcal I$ of $\CSP(\Gamma)$ such that 
it has no solutions but 
$\CheckCycleConsistency$ returns \mbox{``Ok"} on $\mathcal I$.
\end{lem}
\begin{proof}
Consider the following system of linear equations in $\mathbb Z_{p}$.
\begin{equation}\label{LinearEquation}
\left\{
\begin{aligned} %{c}
  x_1+x_2&=x_{3} +\;0\;\\
  x_{3} +\;0\;&=x_4+x_5\\
  x_{4} +\;0\;&=x_1+x_6\\
  x_5+x_6&=x_{2} +\;1\; 
\end{aligned}
\right.
\end{equation}
If we calculate the sum of all equations we will get 
$0=1$, which means that the system does not have a solution.
We can show that the function $\CheckCycleConsistency$ returns \mbox{``Ok"} on this system and this is almost what we need because 
the relation $R$ is very similar 
to $x_{1}+x_{2} = x_{3}+x_{4}$.
Let
\begin{align*}\mathcal I_{0}  = 
((z_{1} = 0)\wedge R(x_1,x_2,x_{3},z_{0}))\wedge 
((z_{2}=0) \wedge R(x_3,z_{2},x_{4},x_{5}))\wedge&\\
((z_{3}=0) \wedge R(x_4,z_{3},x_{1},x_{6}))\wedge
((z_{4}=1) \wedge R(x_5,x_6,x_{2},&z_{4})).
\end{align*}
This is almost an instance of $\CSP(\Gamma)$ and it has no solutions.
Since $R$ is pp-definable over $\Gamma$, 
we can write an equivalent instance 
$\mathcal I$ of $\CSP(\Gamma)$,
that is
$\mathcal I = \mathcal J_{1}\wedge\mathcal J_{2}\wedge\mathcal J_{3}\wedge\mathcal J_{4}$,
where each $\mathcal J_{i}$ is a pp-definition of the corresponding $R$ and the constraint $z_{i} = c$.
Thus, each $\mathcal J_{i}$ corresponds to the $i$-th equation of the system (\ref{LinearEquation}).
We assume that if $i\neq j$ then 
$\mathcal J_{i}$ and $\mathcal J_{j}$ have exactly one common variable and this variable is from the set $X = \{x_{1},\dots,x_{6}\}$.

It remains to show that $\CheckCycleConsistency$ returns 
\mbox{``Ok"} on $\mathcal I$.
We need to prove that 
$\CheckCycleConsistency$ will never reach the situation
when $R_{u,v}=\varnothing$.
Let $V_{i} = \Var(\mathcal J_{i})$ for every $i$.
For $u\in V_{i}$ 
we put 
$S_{u} = \mathcal J_{i}(u)$.
For two variables 
$u,v$ from the same set $V_{i}$ put 
$S_{u,v} = \mathcal J_{i}(u,v)$.
Otherwise, 
if $u\in V_{i}$ and $v\in V_{j}$, 
we put 
$S_{u,v} = S_{u,x}\circ S_{x,v}$, 
where $\{x\} = V_{i}\cap V_{j}$.
Since any two variables of any equation in (\ref{LinearEquation}) can be chosen arbitrary to satisfy the equation, 
we have 
$S_{x_{i},x_{j}} = S_{x_{i}}\times S_{x_{j}}$.

We will prove that 
$R_{u,v}$ 
in $\CheckCycleConsistency$ will always contain 
$S_{u,v}$.
We can check that it is true when we start.
Then, it is sufficient to show that every time we 
calculate $R_{u,v}'$ in $\CheckCycleConsistency$,
it still contains $S_{u,v}$.
This will follow from the fact that 
$S_{u,v}\subseteq S_{u,w}\circ S_{w,v}$
for any $u,v,w\in\Var(\mathcal I)$.
Let us prove this considering 3 cases.


Case 1. If $u,v,w$ are from the same $V_{i}$ then 
it follows from the definition.

Case 2. Otherwise, if $u,w\in V_{\ell}$, $v\in V_{m}$
and $\ell\neq m$, then 
$$S_{u,w}\circ S_{w,v} = S_{u,w}\circ 
S_{w,x_{j}}\circ S_{x_{j},v}
\subseteq \\
S_{u,x_{j}}\circ S_{x_{j},v}=
S_{u,v}
$$


Case 3. Otherwise, if $u\in V_{\ell}$, $w\in V_{m}$, 
$v\in V_{n}$, $\ell\neq m$ and $m\neq n$, then
\begin{align*}
    S_{u,w}\circ S_{w,v} = S_{u,x_{i}}\circ S_{x_{i},w}\circ 
S_{w,x_{j}}\circ S_{x_{j},v}.
\supseteq &\\
S_{u,x_{i}}\circ S_{x_{i},x_{j}}\circ S_{x_{j},v}
=S_{u,x_{i}}\circ 
(S_{x_{i}}\times &S_{x_{j}})\circ S_{x_{j},v}
=S_{u}\times S_{v}.
\end{align*}

Thus, we proved that 
in $\CheckCycleConsistency$ 
we always have 
$R_{u,v}\supseteq S_{u,v}\neq \varnothing$, hence 
$\CheckCycleConsistency$ returns 
\mbox{``Ok"} on $\mathcal I$, which completes the proof.
\end{proof}

Formally, when we reduce the domain of a variable 
of an instance, we may get a relation outside of the constraint language. 
That is why, even if we calculated (for example in 
$\CheckCycleConsistency$) that $x\in B\subsetneq D_{x}$, 
we cannot just reduce the domain of $x$.
%in the instance
%When we check cycle-consistency in 
%$\CheckCycleConsistency$  need 
%to reduce a domain of some variable and therefore 
%we need to restrict the relation. 
To avoid this trouble, 
it is natural to assume that 
for any relation $R\in \Gamma$ and 
any set $D$ pp-definable over $\Gamma$ 
the relation 
$R\cap (A\times\dots\times A\times D\times A\times\dots \times A)$ 
is also from $\Gamma$.
A constraint language satisfying this property will be called 
\emph{unary-closed}.

%For a prime number $p$ by $L_{p}$ we denote the following 
%constraint language on the set $\{0,1,\dots,p-1\}$:
%$L_{p}$ contains the relation $(x_1+x_2=x_3+x_4\mod p)$ 
%and all constant relations.


\begin{thm}
Suppose $\Gamma\subseteq \mathcal R$ is a unary-closed constraint language.
Then the following conditions are equivalent.
\begin{enumerate}
    \item[(1)] $\Gamma$ has a WNU polymorphism of every arity 
    $n\ge 3$;
    \item[(2)] every cycle-consistent instance of $\CSP(\Gamma)$ has a solution;
    \item[(3)] function $\CheckCycleConsistency$ solves $\CSP(\Gamma)$.
%    \item[(4)] there does not exist a prime number $p$ such that 
%    $\CSP(L_{p})$ is polynomially reduced to $\CSP(\Gamma)$,
\end{enumerate}
\end{thm}

\begin{proof}
$(1)\Rightarrow(2)$ is by Theorem \ref{CycleConsistencyImpliesSolutionNonidemp}.

$(2)\Rightarrow(3)$. 
Suppose $\mathcal I$ is an instance of $\CSP(\Gamma)$. 
By Lemma \ref{ProofCycleConsistencyFunction}
if the function 
$\CheckCycleConsistency$ returns \mbox{``No solution"}, 
then it has no solutions.
Assume that it returns
\mbox{``Ok"}.
Then the reduction 
$D^{(\top)}$, defined by 
$D^{(\top)}_{y} = \proj_{1}(R_{y,y})$, is cycle-consistent.
Since $\Gamma$ is unary-closed, 
the instance $\mathcal I^{(\top)}$ is still an instance 
of $\CSP(\Gamma)$ and by (2) it has a solution.
Thus, $\CheckCycleConsistency$ solves $\CSP(\Gamma)$.


$(3)\Rightarrow(1)$. Let us show that 
$\neg(1)\Rightarrow \neg(3)$.
Here we again use the definition of the unary polymorphism $f$, the constraint language 
$\Gamma'$ and the mapping $\Sigma$.
If $\Gamma$ has no a WNU polymorphism $w$ of some arity $m$,
$\Gamma'$ has no a WNU polymorphism $w'$ of some arity $m$
(otherwise,
we would get
$w(x_{1},\dots,x_{m}) = 
f(w(x_{1},\dots,x_{m}))$ is a WNU polymorphism 
of $\Gamma'$.
Applying
Theorem~\ref{CharacterizationOfALLWNUTHM}
to the algebra 
$(f(A),\Pol(\Gamma'))$
we conclude that there exists 
a $p$-WNU-blocker $R$
pp-definable over $\Gamma'$.
By Lemma
\ref{CheckCycleConsistencyFailExample} there exists 
an instance $\mathcal I'$ of $\CSP(\Gamma')$ such that 
$\CheckCycleConsistency$ returns \mbox{``Ok"} on 
it and it does not have a solution.
Then 
$\Sigma(\mathcal I')$ also does not have a solution 
and by Lemma~\ref{CheckConsistencyWorksTheSame}
$\CheckCycleConsistency$ returns \mbox{``Ok"}
on $\Sigma(\mathcal I')$.
\end{proof}

Thus, the cycle-consistency solves the constraint satisfaction problem only if 
the constraint language has a WNU polymorphism 
of every arity $n\ge 3$. 
Moreover, we can prove that 
any local method fails if the constraint language $\Gamma$ has no  WNU polymorphisms of some arity $n\ge 3$. 
In fact, in this case by Theorem~\ref{CharacterizationOfALLWNUTHM}
there exists a $p$-WNU-blocker pp-definable over $\Gamma$
and 
a $p$-WNU-blocker is like a linear equation 
$x_{1}+x_{2} = x_{3} +x_{4}$.
Using this equation and constant relations 
we can express a system of linear equations in $\mathbb Z_{p}$
as an instance of $\CSP(\Gamma)$,
and we know that a system of linear equations cannot be solved locally (see \cite{dsds} for the formal statement).
Hence, we described all the constraint languages that can be solved by local methods. 
Note that 
cycle-consistency is not the weakest consistency that guarantees a solution in this case (see \cite{kozik2016weak} for more details).


 


==> cyclic.tex <==
\subsection{Cyclic term}
A relation $R\subseteq A^{n}$ is called 
\emph{cyclic} 
%if for a cyclic permutation 
%$\sigma:[n]\to[n]$
$R(x_{1},\dots,x_{n}) = 
R(x_{2},\dots,x_{n},x_{1})$.
In this subsection we prove that 
every cyclic relation has 
a constant tuple unless a special blocking relation can be pp-defined from $R$.

\begin{lem}\label{MainNoCyclicLemma}
Suppose 
$\algA$ is a finite idempotent algebra, 
$p$ is a prime number
%$\ge 3$ and 
$R\le \algA^{p}$  is a nonempty cyclic relation.
Then 
\begin{enumerate}
\item[(1)] $(b,b,\dots,b)\in R$ for some $b\in A$, or
\item[(2)] there exists an essentially unary algebra $\alg B\in \HS(\algA)$
with $|B|>1$, or %of size at least 2, or
\item[(3)] there exist $\alg B\in \HS(\algA)$ and $R\le \alg B^{2}$ such that 
$R$ is a graph of a permutation of order $p$ without a fixed point.
\end{enumerate}
\end{lem}

\begin{proof}
We prove by induction on the size of $\algA$.
If $|A|=1$, then condition (1) obviously holds.
Assume that we have 
a subuniverse $B$ of $\algA$ such that 
$R\cap B^{n}\neq\varnothing$.
In this case we may consider 
$R\cap B^{n}$ as an invariant relation on $\alg B$ 
and apply the inductive assumption.
Since a subalgebra of a subalgebra is a subalgebra, 
this completes the proof in this case.
Thus, below we assume that 
$R\cap B^{n}=\varnothing$ for any proper subuniverse $B$ of $\algA$.
We refer to this property as to 
\emph{the empty-property}.
%the inductive assumption.

Since $R$ is cyclic, 
we have 
$\proj_{1}(A)=\dots = \proj_{n}(A)$.
If $\proj_{1}(A)\neq A$, then
$\proj_{1}(A)$ is a proper subuniverse of $\algA$, 
which contradicts the empty-property.
Thus, we assume that $\proj_{1}(A) = A$.
Assume that $\algA$ has a nontrivial congruence $\sigma$.
Then we consider 
the quotient of $R$ modulo $\sigma$, 
that is 
$R/\sigma = 
\{(a_1/\sigma, \dots,a_p/\sigma)\mid 
(a_{1},\dots,a_p)\in R\}$.
By the inductive assumption
$R/\sigma$ has a constant tuple, which gives us an equivalence class (and also a subuniverse) $B$ such that
$R\cap B^{n}\neq\varnothing$. 
Thus, below we assume that 
$\algA$ has no nontrivial congruences.

Then we apply Theorem~\ref{ExistsStrongSubalgebraTHM} and consider 5 cases of this theorem.

\textbf{Cases (1): there exists a nontrivial BA subuniverse $B$ of $\alg A$.}
It is not hard to check that 
$R\cap B^{p}$ is not empty (just apply the absorbing term to all the tuples of $R$).

\textbf{Cases (2)-(3): there exists a strong nontrivial subuniverse $B$ of $\algA$  of type 
$\mathcal T\in\{C,PC\}$.}
Choose a proper $\alg B_{1}\le_{\mathcal T}\algA$ 
so that the relation 
$R\cap (B_1\times A\times\dots\times A)$ contains the maximal number of tuples.
For $i\in[p]$ put 
$B_{i} = \proj_{i}(R\cap (B_1\times A\times\dots\times A))$.
We consider several cases:

Case A. Assume that $B_{i}=A$ for every $i\in\{2,3,\dots,p\}$.
Then $\proj_{1,j}(R)\cap B_1^{2}\neq\varnothing$
for all $j\in[p]$.
Since $R$ is cyclic, 
we get
$\proj_{i,j}(R)\cap B_1^{2}\neq\varnothing$ for all $i,j\in[p]$.
By the empty-property, $R\cap B_1^{p}=\varnothing$.
Choose an inclusion minimal $I\subseteq[p]$ 
such that 
$\proj_{I}(R)\cap B_1^{|I|} = \varnothing$.
We already know that $|I|>2$.
Since $I$ is inclusion-minimal, 
$\proj_{I}(R)$ is a $B_1$-essential relation of arity $|I|>2$, 
which contradicts Theorem~\ref{CommonPropertiesThm}(3).


Case B. There exists $i\in\{2,3,\dots,p\}$ such that 
$B_{i}\neq A$.
Let 
$S = \proj_{1,i}(R)$.
If we restrict the $i$-th variable to $B_{i}$ 
we cannot get a relation having more tuples than
$R\cap (B_{1}\times A\times\dots\times A)$.
Hence, we get exactly the same relation. 
Therefore 
$B_{1}+S = B_{i}$ and $B_{i}-S = B_{1}$.
Therefore $S$ is not linked, 
and unless it is a graph of a permutation, we get a nontrivial 
congruence on $\alg A$, which contradicts our assumption.
Suppose
$\proj_{1,i}(R)$ is a graph of a permutation, 
then the $i$-th coordinate of $R$ is uniquely determined by the
first. 
Since $R$ is cyclic, 
the $j+(i-1)$-th coordinate is uniquely determined by $j$-th
for any $j\in[p]$. 
Since $p$ is prime, 
we can derive that all coordinates are uniquely determined by the first, 
and $\proj_{1,2}(R)$ is also a graph of a permutation.
Moreover, 
$\proj_{1,2}(R) = \proj_{j,j+1}(R)$ for any $j\in[p]$, 
hence the permutation is of order $p$.
If this permutation has a fixed point $c$, 
then $(c,c,\dots,c)\in R$, which is what we need.
Otherwise, 
$\proj_{1,2}(R)$ is a permutation of an order $p$ without a fixed point, that is case (3).

\textbf{Case (4): there exists a congruence $\sigma$ on $\algA$ such that 
$\algA/\sigma$ is $q$-affine.}
Since we assumed that $\algA$ doesn't have a nontrivial congruence, 
$\algA$ is $q$-affine.
Suppose $\oplus$ and $\ominus$ are from the definition of 
$q$-affine, and 
$c_0$ and $c_{1}$ are the elements of $A$ corresponding to 
$(0,\dots,0)$ and $(1,\dots,1)$, respectively.
If $q=p$, 
then substituting $c_0$ and $c_1$ into the 
relation 
$x_{1}\oplus x_2 = x_{3}\oplus x_{4}$
for $x_2$ and $x_{4}$, respectively, 
we get a binary relation, that is a graph of a permutation of order $p$ without a fixed point.

Suppose $q\neq p$.
%Consider an operation 
%$m(x,y,z) = x\ominus y\oplus z$.
Choose $k$ such that 
$q$ divides $(k\cdot p-1)$.
Let %\ominus x_1\oplus x_4
\begin{align*}
t(x_{1},\dots,x_{kp}) = 
x_1\ominus x_{1}\oplus x_2 \ominus x_1\oplus x_3
 \ominus \dots \ominus x_1\oplus 
x_{kp}=&
\\
x_1\oplus x_2\oplus& \dots\oplus x_{kp}
.
\end{align*}
Choose a tuple $(a_{1},\dots,a_{p})\in R$,
for every $i$
by $\alpha_{i}$ we denote the tuple 
$(a_{i},\dots,a_{p},a_{1}\dots,a_{i-1})\in R$.
Then a constant tuple of $R$ can be defined  by 
$$t(\alpha_{1},\dots,\alpha_{p},\alpha_{1},\dots,\alpha_{n},\dots,\alpha_{1},\dots,\alpha_{p}).$$

\textbf{Case (5): there exists a nontrivial CBT subuniverse $B$.}
If $B$ is also a binary absorbing subuniverse, 
then it is the case (1) of Theorem~\ref{ExistsStrongSubalgebraTHM}.
Otherwise, by Lemma~\ref{CBTNonAbsorbing}
there exists essentially unary algebra $\alg B\in \HS(\algA)$.
\end{proof}


We will use the following facts from \cite{cyclicproperties}.

\begin{lem}\cite[Proposition 2.2]{cyclicproperties}\label{cyclicfactor}
Let $C(\algA)$ be the set of integers $n$ 
such that $\algA$ has a cyclic term of arity $n$.
Then 
\begin{itemize}
    \item if $n\in C(\algA)$ and $1<k|n$, then 
    $k\in C(\algA)$.
    \item if $m,n\in C(\algA)$ then $m\cdot n\in C(\algA)$.
\end{itemize}
\end{lem}

\begin{lem}\cite[Lemma 2.4]{cyclicproperties}\label{cyclictuplereduction}
Let $\algA$ be a finite idempotent algebra, 
$n\ge 2$. The following are equivalent:
\begin{enumerate}
    \item $\algA$ has an $n$-ary cyclic term operation.
    \item for any 
    $(a_1,\dots,a_n)\in A^{n}$ there exists a term operation $t$
    such that 
    $t(a_{i},\dots,a_{n},a_{1},\dots,a_{n-1})$ is a constant for all $i\in[n]$.
\end{enumerate}
\end{lem}


\begin{lem}\label{NoCylcicLemma}
Suppose 
$\algA$ is a finite idempotent algebra having a cyclic term operation.
Then 
$\algA$ has a cyclic term operation of arity $n\ge 2$ if and only if 
there not exist 
$\alg B\in \HS(\algA)$ and $R\le \alg B^{2}$ such that 
$R$ is a graph of a permutation of a prime order $p$ without a fixed point, where $p$ divides $n$.
\end{lem}
\begin{proof}
By Lemma~\ref{cyclicfactor} it is sufficient to prove this lemma only for prime $n$.

$\Rightarrow$. It is easy to check that 
a cyclic operation of arity $n$ cannot preserve a 
graph of permutation of order $n$ without a fixed point.

$\Leftarrow$. 
By Lemma~\ref{cyclictuplereduction} it is sufficient to find 
a term operation $t$
for any $(a_1,\dots,a_n)\in A^{n}$ 
    such that 
    $t(a_{i},\dots,a_{n},a_{1},\dots,a_{n-1})$ is constant for all $i\in[n]$.
    Let $R$ be the relation generated from 
    the $n$ tuples of the form
    $(a_{i},\dots,a_{n},a_{1},\dots,a_{n-1})$, where $i=1,2,\dots,n$.
    Obviously, the obtained relation is cyclic, therefore
    by Lemma~\ref{MainNoCyclicLemma}
    $R$ should have a constant tuple. 
%Then by Lemma~\ref{cyclictuplereduction} there exists a cyclic operation of arity $n$.
\end{proof}

